C3PO: Towards a complete census of co-moving pairs of stars. I. High precision stellar parameters for 250 stars

We conduct a line-by-line differential analysis of a sample of 125 co-moving pairs of stars (dwarfs and subgiants near solar metallicity). We obtain high precision stellar parameters with average uncertainties in effective temperature, surface gravity and metallicity of 16.5 K, 0.033 dex and 0.014 dex, respectively. We classify the co-moving pairs of stars into two groups, chemically homogeneous (conatal; |Delta[Fe/H]| $\le$ 0.04 dex) and inhomogeneous (non-conatal), and examine the fraction of chemically homogeneous pairs as a function of separation and effective temperature. The four main conclusions from this study are: (1) A spatial separation of \ds = 10$^6$ AU is an approximate boundary between homogeneous and inhomogeneous pairs of stars, and we restrict our conclusions to only consider the 91 pairs with \ds $\le$ 10$^6$ AU; (2) There is no trend between velocity separation and the fraction of chemically homogeneous pairs in the range \dv $\le$ 4 \kms; (3) We confirm that the fraction of chemically inhomogeneous pairs increases with increasing \teff\ and the trend matches a toy model of that expected from planet ingestion; (4) Atomic diffusion is not the main cause of the chemical inhomogeneity. A major outcome from this study is a sample of 56 bright co-moving pairs of stars with chemical abundance differences $\leq$ 0.02 dex (5\%) which is a level of chemical homogeneity comparable to that of the Hyades open cluster. These important objects can be used, in conjunction with star clusters and the \gaia\ ``benchmark'' stars, to calibrate stellar abundances from large-scale spectroscopic surveys.

==> tab1.full.tex <==
\begin{table*}
	\caption{Program stars and observing details.}
	\label{tab:obs}
	\begin{tabular}{llcclrcccccc}
	\hline
  Pair ID &
  Gaia\_ID\_ref &
  G\_ref &
  bp\_rp\_ref &
  Gaia\_ID\_obj &
  G\_obj &
  bp\_rp\_obj &
  $\Delta$ s ($\log$ AU) &
  $\Delta$ v (\kms) &
  Anom &
  Observed \\
\hline
   1 &     55780840513067392 &   8.373 &  0.783 &     55780840513308160 &   9.321 &  0.715 &   5.19 &   1.50 &  Y &  C,D \\ 
   2 &    627699888238838528 &   8.216 &  0.870 &    627699888238838272 &   7.458 &  0.742 &   4.29 &   0.51 &  N &    F \\ 
   3 &    692119656035933568 &   8.121 &  0.732 &    692120029700390912 &   8.144 &  0.738 &   4.81 &   0.75 &  N &    G \\ 
   4 &    704994524881597184 &   9.851 &  0.734 &    704994524881597056 &   9.855 &  0.733 &   4.90 &   0.78 &  N &    F \\ 
   5 &    736173925863826944 &   9.195 &  0.892 &    736174028943041920 &   9.206 &  0.884 &   4.40 &   0.80 &  Y &    G \\ 
   6 &    775037328283498624 &   9.443 &  0.786 &    741830466512452736 &   9.825 &  0.860 &   6.47 &   0.56 &  N &    G \\ 
   7 &    773252069293117696 &   8.973 &  0.786 &    773252069293612672 &   9.714 &  0.764 &   5.94 &   1.97 &  N &    G \\ 
   8 &    844865117036623232 &   7.556 &  0.802 &    844865117036622976 &   8.003 &  0.951 &   5.83 &   2.90 &  Y &    G \\ 
   9 &   1549927395024812672 &   8.225 &  0.741 &    844865117036623232 &   7.556 &  0.802 &   6.71 &   0.62 &  Y &    G \\ 
  10 &   1038148059924483328 &   8.701 &  0.775 &   1040472083909088128 &   9.317 &  0.906 &   6.19 &   1.68 &  Y &    G \\ 
  11 &   1167718049194619136 &   7.378 &  0.842 &   1167718049194619264 &   7.189 &  0.807 &   3.90 &   1.69 &  N &    C \\ 
  12 &   1519964225698087680 &   9.487 &  0.843 &   1519964294418209664 &   9.516 &  0.822 &   5.86 &   1.92 &  N &    G \\ 
  13 &   1552368070320568192 &   9.368 &  0.796 &   1552365046663591552 &   9.651 &  0.832 &   4.46 &   1.78 &  N &    G \\ 
  14 &   2331411774161459328 &   9.655 &  0.790 &   2331411778456143232 &   9.573 &  0.778 &   4.79 &   1.00 &  N &    A \\ 
  15 &   2356290256259997696 &   7.856 &  0.808 &   2356080043380354816 &   8.131 &  0.750 &   5.17 &   0.44 &  Y &    B \\ 
  16 &   2632792584258400640 &   9.629 &  0.950 &   2366265678581766272 &   9.165 &  0.857 &   6.63 &   0.68 &  N &    D \\ 
  17 &   2388618372016602240 &   9.446 &  0.769 &   2388618372016602368 &   9.898 &  0.852 &   4.60 &   0.80 &  N &    D \\ 
  18 &   5030721964337409536 &   9.071 &  0.873 &   2456617393759254400 &   8.644 &  0.744 &   6.80 &   0.82 &  Y &    B \\ 
  19 &   2398083032532932480 &   9.439 &  0.749 &   2611083178139983744 &   9.020 &  0.676 &   6.66 &   1.35 &  Y &    D \\ 
  20 &   2731708498584058368 &   8.234 &  0.912 &   2630545461664620288 &   9.114 &  1.038 &   6.59 &   0.62 &  Y &    D \\ 
  21 &   2630906926112239616 &   9.170 &  0.837 &   2630937059602783616 &   8.499 &  0.720 &   4.88 &   0.94 &  N &    B \\ 
  22 &   2638615189818036736 &   8.042 &  0.773 &   2638615189818036608 &   8.401 &  0.835 &   4.23 &   1.30 &  N &    B \\ 
  23 &   6899460856141456384 &   8.650 &  0.669 &   2670687222445537152 &   9.600 &  0.771 &   6.38 &   1.40 &  Y &    D \\ 
  24 &   2713861882972485504 &   8.929 &  0.698 &   2713872019095313536 &   8.623 &  0.660 &   5.31 &   0.72 &  N &    C \\ 
  25 &   2815476857825953408 &   9.389 &  0.822 &   2714025229168797696 &   9.156 &  0.693 &   6.70 &   1.17 &  Y &    C \\ 
  26 &   2919963104221492480 &   8.909 &  0.987 &   2919963104216198528 &   9.014 &  1.050 &   4.06 &   1.73 &  N &    H \\ 
  27 &   3002531548383047296 &   9.262 &  1.043 &   3002343871195786496 &   9.545 &  1.127 &   3.86 &   0.46 &  N &    H \\ 
  28 &   3084652044636398976 &   9.953 &  0.949 &   3084652044636399104 &   9.357 &  0.838 &   4.66 &   1.41 &  Y &    F \\ 
  29 &   3092798291923831296 &   9.605 &  0.862 &   3085625554805818240 &   9.380 &  0.804 &   6.60 &   0.92 &  Y &    G \\ 
  30 &   3170394607068638336 &   9.505 &  0.765 &   3170300942420466176 &   9.291 &  0.764 &   4.82 &   0.79 &  N &    F \\ 
  31 &   3018965776882444416 &   9.231 &  0.818 &   3183053112639796352 &   8.873 &  0.772 &   6.62 &   0.71 &  Y &    E \\ 
  32 &   3208713618088140160 &   9.225 &  0.740 &   3208713618088139520 &   9.510 &  0.720 &   4.94 &   1.74 &  N &    H \\ 
  33 &   3230677565443833088 &   7.361 &  0.727 &   3230677874682668672 &   7.369 &  0.731 &   4.51 &   0.43 &  Y &  C,D \\ 
  34 &   3285218255623808640 &   6.778 &  0.860 &   3285218186904332288 &   6.175 &  0.743 &   3.64 &   1.21 &  N &  C,D \\ 
  35 &   3285755951169814656 &   9.102 &  0.688 &   3285744612456149888 &   9.403 &  0.750 &   5.00 &   0.36 &  N &    D \\ 
  36 &   3288572968680438528 &   7.977 &  1.028 &   3288572968680438912 &   8.123 &  1.066 &   3.80 &   0.72 &  N &  C,D \\ 
  37 &   3306104544145237504 &   8.573 &  0.801 &   3334853612116832128 &   8.591 &  0.697 &   6.77 &   0.91 &  Y &    F \\ 
  38 &   3359820016490648576 &   7.667 &  0.733 &   3359808231100381312 &   7.572 &  0.716 &   4.38 &   1.99 &  Y &  E,F \\ 
  39 &   3451267120128948992 &   8.279 &  0.902 &   3451266742171824640 &   8.526 &  0.959 &   4.01 &   0.57 &  N &    F \\ 
  40 &   3457532373603470336 &   9.222 &  0.713 &   3456111877595120256 &   9.926 &  0.810 &   6.24 &   0.77 &  Y &    F \\ 
  41 &   3613454637229633664 &  10.804 &  0.788 &   3613454637229634176 &  10.442 &  0.815 &   5.28 &   1.37 &  N &    A \\ 
  42 &   3616756294553180160 &   9.145 &  0.838 &   3616756294553180288 &   9.620 &  0.936 &   4.22 &   2.06 &  N &    A \\ 
  43 &   3639520621950395904 &   7.420 &  0.741 &   3639520621950395776 &   7.430 &  0.743 &   4.36 &   1.37 &  N &    A \\ 
  44 &   3717329177197429376 &   9.925 &  0.728 &   3717329172901660160 &   9.685 &  0.699 &   4.98 &   0.81 &  N &    H \\ 
  45 &   3749791055416743552 &   9.286 &  0.916 &   3749791158495959552 &   9.019 &  0.869 &   4.45 &   0.45 &  N &    H \\ 
  46 &   3759082066110510208 &   9.758 &  0.760 &   3759082066110510080 &   9.631 &  0.798 &   5.72 &   1.87 &  N &    H \\ 
  47 &   3830034685322011136 &   9.494 &  0.675 &   3830034479163581312 &   8.897 &  0.703 &   5.22 &   1.32 &  N &    H \\ 
  48 &    613140808098832000 &   9.807 &  0.860 &   3836997136546164736 &   9.544 &  0.777 &   6.46 &   0.61 &  Y &    G \\ 
  49 &   3898778969789498880 &   9.702 &  0.729 &   3898778901070021504 &   9.040 &  0.659 &   4.76 &   0.57 &  N &    H \\ 
  50 &   3945118643256370688 &   8.345 &  0.938 &   3945118265299248128 &   7.979 &  0.858 &   4.17 &   0.41 &  N &    G \\ 
  51 &   3975223065466473216 &   8.235 &  0.890 &   3975129194660883328 &   8.039 &  0.848 &   4.02 &   0.31 &  Y &    G \\ 
  52 &   4024887730814401280 &   9.893 &  0.690 &   4024886425144354816 &   9.787 &  0.680 &   5.20 &   0.61 &  N &    G \\ 
  53 &   4269938532999515008 &   9.328 &  0.844 &   4104278208452966912 &   9.493 &  0.806 &   6.73 &   0.96 &  Y &    D \\ 
  54 &   6643680401021447296 &   9.452 &  0.775 &   4174091454408295680 &   9.394 &  0.841 &   7.26 &   1.35 &  Y &    A \\ 
  55 &   4193020582174571264 &   9.403 &  0.743 &   4193020582169053056 &   9.044 &  0.659 &   4.98 &   1.54 &  N &    C \\ 
  56 &   4197023904014523776 &   8.571 &  0.736 &   4197023904013455872 &   9.079 &  0.832 &   4.38 &   0.90 &  N &    B \\ 
  57 &   4199387544795379968 &   9.368 &  0.780 &   4199387544795378176 &   9.367 &  0.781 &   4.77 &   0.80 &  N &    C \\ 
  58 &   4235731867269159680 &   8.896 &  0.737 &   4235732073427592704 &   8.722 &  0.722 &   4.72 &   1.17 &  N &    A \\ 
  59 &   4240626686883261184 &   8.551 &  1.034 &   4240625896609242624 &   8.692 &  1.066 &   4.52 &   0.71 &  Y &    C \\ 
  60 &   4249652783985617920 &   7.859 &  0.828 &   4249652990144051840 &   7.556 &  0.857 &   4.60 &   0.95 &  N &    C \\ 
  61 &   4499162449416966272 &   8.357 &  0.718 &   4287378367995943680 &   8.060 &  0.759 &   6.67 &   0.93 &  Y &    C \\ 
  62 &   4343064508746082304 &   7.796 &  1.010 &   4343064577465522816 &   7.277 &  0.893 &   3.73 &   0.80 &  Y &    B \\ 
  63 &   4360581000283303936 &   9.890 &  0.854 &   4360581000283303552 &   9.724 &  0.821 &   4.61 &   1.53 &  N &    A \\ 
  64 &   6236816675902817536 &   8.594 &  0.866 &   4383238052280567680 &   8.077 &  0.724 &   6.74 &   0.53 &  Y &    B \\ 
  65 &   1198060172076731520 &   8.534 &  0.821 &   4421376193636525184 &   9.021 &  0.895 &   6.51 &   0.76 &  Y &    C \\ 
  66 &   4461273278722817792 &   9.373 &  0.962 &   4461273072564386816 &   8.911 &  0.872 &   4.44 &   0.30 &  N &    D \\ 
  67 &   4464207428577214464 &   7.263 &  0.938 &   4464207428579939840 &   7.182 &  0.920 &   3.64 &   1.79 &  N &    D \\ 
  68 &   4648549830108994816 &   9.497 &  0.670 &   4648549830108995200 &   9.379 &  0.668 &   4.93 &   0.96 &  Y &    H \\ 
  69 &   4666907551119833984 &   7.286 &  0.771 &   4666907516760096512 &   7.439 &  0.752 &   4.06 &   0.41 &  Y &  C,D \\ 
  70 &   4677970179988001280 &   9.694 &  0.765 &   4677970179987090304 &   9.867 &  0.804 &   4.55 &   1.34 &  N &    H \\ 
  71 &   4803965455094278528 &   9.676 &  0.757 &   4805634616824440192 &   9.933 &  0.819 &   6.22 &   0.36 &  N &    H \\ 
  72 &   4867855155206070784 &   9.865 &  0.972 &   4813691219557127808 &   9.201 &  0.841 &   6.29 &   1.49 &  N &    D \\ 
  73 &   4837828175549438080 &   9.677 &  0.722 &   4837828179846041728 &   9.806 &  0.743 &   4.51 &   1.07 &  N &    H \\ 
  74 &   4857866023347844608 &   9.168 &  0.732 &   4857866019051550976 &   8.667 &  0.664 &   4.35 &   0.80 &  Y &    H \\ 
  75 &   4873226853623529856 &   8.676 &  0.824 &   4873223623808123136 &   8.676 &  0.819 &   4.56 &   0.66 &  N &    H \\ 
  76 &   4940794488850252928 &   9.146 &  0.678 &   4940794866807373952 &   8.995 &  0.670 &   4.58 &   0.78 &  Y &    H \\ 
  77 &   5195685713943687168 &   9.726 &  0.729 &   5195685713943683072 &   9.611 &  0.716 &   4.75 &   0.55 &  Y &    H \\ 
  78 &   5255388783050605824 &   9.658 &  1.002 &   5255388783050603136 &   9.632 &  0.996 &   4.20 &   0.75 &  N &    H \\ 
  79 &   5296896240321814144 &   9.637 &  1.063 &   5296896205962076416 &   9.300 &  0.977 &   4.33 &   1.29 &  N &    H \\ 
  80 &   5401057271783266432 &   9.779 &  0.750 &   5401057271781148032 &   9.961 &  0.745 &   4.93 &   0.56 &  N &    H \\ 
  81 &   5484928568505017472 &   8.052 &  0.751 &   5484928534145279744 &   8.918 &  0.730 &   4.88 &   0.83 &  N &    H \\ 
  82 &   5485115519841798912 &   8.573 &  0.744 &   5485115588561239808 &   8.852 &  0.770 &   4.19 &   0.75 &  N &    E \\ 
  83 &   5595858262287843840 &   8.560 &  0.827 &   5595858159201264768 &   9.502 &  0.872 &   4.38 &   1.05 &  N &    H \\ 
  84 &   5744680768862271872 &   9.021 &  0.819 &   5744680768862271616 &   9.783 &  0.696 &   5.40 &   1.52 &  N &    G \\ 
  85 &   5807733500118617984 &  10.192 &  0.859 &   5778002293379364992 &  10.235 &  0.924 &   6.70 &   1.18 &  Y &    A \\ 
  86 &   5778208829765876864 &   9.959 &  0.751 &   5778208829765877376 &  10.231 &  0.759 &   5.19 &   1.18 &  N &    A \\ 
  87 &   5798991008295109120 &  10.447 &  0.893 &   5798991008295120896 &  10.315 &  0.883 &   5.51 &   1.46 &  N &    A \\ 
  88 &   5821555284685890304 &   8.751 &  0.663 &   5825293319323469824 &   8.499 &  0.736 &   6.47 &   1.48 &  Y &    C \\ 
  89 &   5863709946382545280 &   8.415 &  0.698 &   5863709946382541952 &   9.004 &  0.772 &   4.30 &   0.34 &  N &    H \\ 
  90 &   5877155289930033024 &   9.504 &  0.833 &   5877155289930029184 &   9.670 &  0.844 &   4.90 &   1.08 &  Y &    A \\ 
  91 &   5897704951769034368 &  10.127 &  0.838 &   5897785667103983616 &  10.277 &  0.800 &   6.19 &   1.07 &  Y &    A \\ 
  92 &   2598586816173411200 &   7.160 &  0.691 &   5976865876277242112 &   7.540 &  0.783 &   7.06 &   0.86 &  Y &    A \\ 
  93 &   6003429213889816832 &   6.874 &  0.769 &   6003429424356691584 &   7.444 &  0.871 &   3.75 &   0.96 &  N &    B \\ 
  94 &   6004256909931771136 &   8.481 &  0.969 &   6004256802548180736 &   8.270 &  0.928 &   4.03 &   0.82 &  N &    A \\ 
  95 &   6099322403253174016 &  10.387 &  0.892 &   6118406798373150848 &  10.253 &  0.919 &   6.55 &   1.96 &  Y &    A \\ 
  96 &   6193279279612173952 &   8.468 &  1.116 &   6193280031230266752 &   8.516 &  1.123 &   4.15 &   1.24 &  N &    H \\ 
  97 &   6208919660724640896 &  10.275 &  1.032 &   6208919660723526272 &   9.998 &  0.970 &   4.91 &   1.47 &  Y &    A \\ 
  98 &   5906633952564270848 &   7.556 &  0.904 &   6213644846302305536 &   7.333 &  0.917 &   6.29 &   4.37 &  Y &    A \\ 
  99 &   6214634887804201728 &   9.865 &  0.823 &   6214634887804233088 &  10.000 &  0.843 &   4.63 &   1.04 &  N &    A \\ 
 100 &   6224633983987510528 &   8.285 &  0.790 &   6224633983987511552 &   8.270 &  0.785 &   4.29 &   1.67 &  N &    A \\ 
 101 &   6274656261191532160 &   9.661 &  0.772 &   6274653310550270592 &   9.842 &  0.759 &   5.02 &   2.05 &  Y &    H \\ 
 102 &   6295940298044771072 &   9.556 &  0.780 &   6295940302339553664 &   9.808 &  0.734 &   5.54 &   0.69 &  Y &    H \\ 
 103 &   6317420219765757440 &   9.344 &  0.777 &   6317420224061370624 &   9.493 &  0.783 &   4.91 &   1.68 &  N &    D \\ 
 104 &   6369977773223661184 &  10.443 &  0.903 &   6369977876303556736 &  10.393 &  0.778 &   5.42 &   0.45 &  Y &    A \\ 
 105 &   6740764911228220288 &   9.250 &  0.900 &   6381091636756147200 &   9.216 &  0.957 &   7.02 &   1.24 &  Y &    A \\ 
 106 &   6463958151650359040 &   7.533 &  0.842 &   6409419145097654016 &   7.736 &  0.765 &   6.37 &   1.69 &  N &    B \\ 
 107 &   6709875880094622720 &   9.153 &  0.839 &   6420597089545019776 &   9.033 &  0.939 &   6.82 &   1.04 &  N &    A \\ 
 108 &   6463958151650359040 &   7.533 &  0.842 &   6463958151650358784 &   7.712 &  0.874 &   3.87 &   1.84 &  N &    B \\ 
 109 &   6463958151650358784 &   7.712 &  0.874 &   6463958151650359040 &   7.533 &  0.842 &   3.87 &   1.84 &  N &    C \\ 
 110 &   6471977542786978688 &   8.882 &  0.778 &   6471977336628547968 &   9.867 &  0.911 &   4.44 &   1.31 &  N &    D \\ 
 111 &   6473063860275183616 &   8.868 &  0.678 &   6472230636619614464 &   8.950 &  0.672 &   6.78 &   0.50 &  Y &    B \\ 
 112 &   6497943781186827264 &  10.068 &  0.830 &   6497943781187251072 &  10.483 &  0.906 &   5.14 &   0.66 &  Y &    A \\ 
 113 &   6518007050894577664 &   9.994 &  0.759 &   6518006565562564352 &   9.810 &  0.743 &   5.05 &   0.68 &  Y &    A \\ 
 114 &   2328250334633289856 &   8.835 &  0.985 &   6527965258988306304 &   8.606 &  0.919 &   6.50 &   1.76 &  Y &    B \\ 
 115 &   6570797524722448896 &   9.984 &  1.070 &   6570796871887419648 &   9.372 &  0.956 &   4.60 &   0.35 &  N &    D \\ 
 116 &   6644929416166727680 &   9.368 &  0.801 &   6644929656684912512 &   9.501 &  0.797 &   4.70 &   1.07 &  Y &    A \\ 
 117 &   6666179333798782976 &   9.527 &  1.035 &   6666179127640352512 &   9.631 &  1.066 &   3.96 &   1.22 &  N &    A \\ 
 118 &   6673293174030454400 &  10.257 &  0.981 &   6673292933512285312 &   9.894 &  0.915 &   4.81 &   0.36 &  N &    A \\ 
 119 &   6673835645579910016 &   8.246 &  0.801 &   6673835611220171904 &   8.999 &  0.743 &   4.56 &   0.27 &  Y &    B \\ 
 120 &   6743004646477330560 &   9.289 &  0.968 &   6743004650775553280 &   9.461 &  1.005 &   4.02 &   1.61 &  Y &    A \\ 
 121 &   6805776216277879808 &   9.238 &  0.957 &   6805776211983950080 &   9.486 &  1.006 &   4.42 &   3.05 &  N &    A \\ 
 122 &   6827651171911478272 &   9.350 &  1.059 &   6827651373773901568 &   9.346 &  1.047 &   4.00 &   1.76 &  Y &    C \\ 
 123 &   5767612458250649216 &   7.492 &  0.761 &   6866542478736575616 &   7.147 &  0.738 &   7.18 &   1.78 &  Y &    A \\ 
 124 &   6868438517820721152 &   8.845 &  0.694 &   6868432504866186368 &   9.423 &  0.727 &   4.90 &   0.82 &  Y &    C \\ 
 125 &   6900155614347675648 &   9.653 &  0.757 &   6889841508084452096 &   9.031 &  0.684 &   6.40 &   1.30 &  Y &    D \\ 
	\hline
	\end{tabular}
	\\ 
	A = Magellan, June 2019; B = Magellan, 13 Aug 2021; C = Magellan, 26 Aug 2021; D = Magellan, 27 Aug 2021; E = Magellan, 11 Nov 2021; F = Keck, 20 Dec 2021; G = Keck, 16 Jan 2022; H = ESO, Period 108. \\
    (Recall that while the labels ``reference'' and ``object'' are interchangeable, we retain the distinction here to signify the manner in which the differential analysis was performed; see Sec 3 for details.) \\ 
	This table is published in its entirety in the electronic edition of the paper. A portion is shown here for guidance regarding its form and content.
\end{table*}



==> tab3.full.tex <==
\begin{table*}
	\caption{Stellar parameters.}
	\label{tab:param}
	\begin{tabular}{llccrlccccrc}
	\hline
  Pair ID &
  Gaia\_ID\_ref &
  \teff &
  \logg &
  [Fe/H] &
  Gaia\_ID\_obj &
  \teff &
  $\sigma$\teff &
  \logg &
  $\sigma$\logg &
  [Fe/H] &
  $\sigma$[Fe/H] \\ 
  &
  (ref) &
  (ref) &
  (ref) &
  &
  (obj) &
  (obj) &
  (obj) &
  (obj) &
  (obj) &
  (obj) \\ 
\hline
   1 &     55780840513067392 & 5986 &  3.970 &   0.082 &     55780840513308160 & 6164 &   10 &  4.240 &  0.024 &   0.014 &  0.008 \\ 
   2 &    627699888238838528 & 5579 &  4.540 &  -0.195 &    627699888238838272 & 6021 &   18 &  4.530 &  0.032 &  -0.220 &  0.015 \\ 
   3 &    692119656035933568 & 6003 &  4.560 &  -0.355 &    692120029700390912 & 6004 &   12 &  4.600 &  0.022 &  -0.333 &  0.009 \\ 
   4 &    704994524881597184 & 6034 &  4.490 &  -0.289 &    704994524881597056 & 6070 &   13 &  4.530 &  0.023 &  -0.291 &  0.008 \\ 
   5 &    736173925863826944 & 5589 &  4.520 &   0.159 &    736174028943041920 & 5615 &   10 &  4.530 &  0.017 &   0.124 &  0.007 \\ 
   6 &    775037328283498624 & 5836 &  4.470 &  -0.027 &    741830466512452736 & 5628 &   16 &  4.480 &  0.034 &  -0.027 &  0.015 \\ 
   7 &    773252069293117696 & 5979 &  4.080 &   0.215 &    773252069293612672 & 6036 &    8 &  4.360 &  0.021 &   0.219 &  0.008 \\ 
   8 &    844865117036623232 & 5900 &  4.450 &   0.249 &    844865117036622976 & 5620 &   29 &  4.510 &  0.044 &   0.086 &  0.021 \\ 
   9 &   1549927395024812672 & 6084 &  4.490 &   0.126 &    844865117036623232 & 5902 &   11 &  4.450 &  0.030 &   0.251 &  0.015 \\ 
  10 &   1038148059924483328 & 5992 &  4.570 &   0.068 &   1040472083909088128 & 5456 &   14 &  4.510 &  0.024 &  -0.216 &  0.011 \\ 
  11 &   1167718049194619136 & 5776 &  4.490 &   0.125 &   1167718049194619264 & 5894 &   13 &  4.480 &  0.026 &   0.137 &  0.013 \\ 
  12 &   1519964225698087680 & 5779 &  4.040 &   0.108 &   1519964294418209664 & 5888 &   17 &  4.110 &  0.038 &   0.121 &  0.016 \\ 
  13 &   1552368070320568192 & 5946 &  4.450 &   0.125 &   1552365046663591552 & 5795 &   19 &  4.490 &  0.031 &   0.130 &  0.015 \\ 
  14 &   2331411774161459328 & 5877 &  4.410 &   0.140 &   2331411778456143232 & 5920 &    9 &  4.400 &  0.026 &   0.137 &  0.013 \\ 
  15 &   2356290256259997696 & 5823 &  4.070 &  -0.107 &   2356080043380354816 & 6021 &    7 &  4.230 &  0.017 &  -0.066 &  0.007 \\ 
  16 &   2632792584258400640 & 5394 &  4.550 &  -0.036 &   2366265678581766272 & 5665 &   11 &  4.530 &  0.022 &  -0.058 &  0.012 \\ 
  17 &   2388618372016602240 & 5971 &  4.540 &   0.003 &   2388618372016602368 & 5668 &   13 &  4.550 &  0.022 &   0.025 &  0.011 \\ 
  18 &   5030721964337409536 & 5659 &  4.310 &   0.296 &   2456617393759254400 & 5996 &   20 &  4.430 &  0.049 &  -0.059 &  0.019 \\ 
  19 &   2398083032532932480 & 6092 &  4.550 &  -0.018 &   2611083178139983744 & 6327 &   17 &  4.490 &  0.029 &   0.019 &  0.013 \\ 
  20 &   2731708498584058368 & 5510 &  4.490 &   0.162 &   2630545461664620288 & 5204 &   26 &  4.530 &  0.033 &   0.080 &  0.017 \\ 
  21 &   2630906926112239616 & 5745 &  4.490 &   0.146 &   2630937059602783616 & 6132 &   11 &  4.440 &  0.032 &   0.139 &  0.014 \\ 
  22 &   2638615189818036736 & 5953 &  4.450 &   0.153 &   2638615189818036608 & 5748 &    8 &  4.480 &  0.016 &   0.163 &  0.009 \\ 
  23 &   6899460856141456384 & 6360 &  3.910 &   0.022 &   2670687222445537152 & 5934 &   26 &  4.060 &  0.053 &  -0.202 &  0.017 \\ 
  24 &   2713861882972485504 & 6215 &  4.360 &  -0.179 &   2713872019095313536 & 6361 &   18 &  4.260 &  0.041 &  -0.194 &  0.013 \\ 
  25 &   2815476857825953408 & 5791 &  4.420 &  -0.065 &   2714025229168797696 & 6352 &   21 &  4.410 &  0.053 &   0.181 &  0.019 \\ 
  26 &   2919963104221492480 & 5305 &  4.535 &   0.056 &   2919963104216198528 & 5247 &   16 &  4.535 &  0.019 &   0.046 &  0.013 \\ 
  27 &   3002531548383047296 & 5099 &  4.555 &  -0.595 &   3002343871195786496 & 4929 &   19 &  4.540 &  0.031 &  -0.625 &  0.018 \\ 
  28 &   3084652044636398976 & 5400 &  4.470 &   0.170 &   3084652044636399104 & 5745 &   16 &  4.520 &  0.025 &   0.116 &  0.016 \\ 
  29 &   3092798291923831296 & 5613 &  4.540 &  -0.146 &   3085625554805818240 & 5840 &   29 &  4.480 &  0.056 &   0.039 &  0.025 \\ 
  30 &   3170394607068638336 & 5929 &  4.320 &  -0.249 &   3170300942420466176 & 5941 &   11 &  4.260 &  0.031 &  -0.258 &  0.010 \\ 
  31 &   3018965776882444416 & 5762 &  4.470 &  -0.117 &   3183053112639796352 & 5950 &   12 &  4.510 &  0.022 &   0.139 &  0.012 \\ 
  32 &   3208713618088140160 & 6159 &  4.265 &  -0.104 &   3208713618088139520 & 6104 &   18 &  4.355 &  0.046 &  -0.106 &  0.012 \\ 
  33 &   3230677565443833088 & 6018 &  4.050 &  -0.272 &   3230677874682668672 & 6053 &   12 &  4.120 &  0.026 &  -0.218 &  0.011 \\ 
  34 &   3285218255623808640 & 5648 &  4.490 &  -0.028 &   3285218186904332288 & 6042 &   12 &  4.440 &  0.031 &  -0.020 &  0.012 \\ 
  35 &   3285755951169814656 & 6224 &  4.410 &  -0.063 &   3285744612456149888 & 6036 &   17 &  4.490 &  0.029 &  -0.057 &  0.011 \\ 
  36 &   3288572968680438528 & 5224 &  4.530 &   0.111 &   3288572968680438912 & 5153 &   16 &  4.560 &  0.023 &   0.112 &  0.008 \\ 
  37 &   3306104544145237504 & 5882 &  4.550 &   0.026 &   3334853612116832128 & 6273 &   20 &  4.510 &  0.032 &   0.107 &  0.016 \\ 
  38 &   3359820016490648576 & 6004 &  4.430 &  -0.349 &   3359808231100381312 & 6094 &   21 &  4.470 &  0.048 &  -0.512 &  0.014 \\ 
  39 &   3451267120128948992 & 5525 &  4.540 &  -0.023 &   3451266742171824640 & 5357 &    9 &  4.530 &  0.013 &  -0.017 &  0.011 \\ 
  40 &   3457532373603470336 & 6219 &  4.400 &   0.039 &   3456111877595120256 & 5928 &   21 &  4.560 &  0.040 &   0.219 &  0.024 \\ 
  41 &   3613454637229633664 & 6113 &  4.410 &   0.183 &   3613454637229634176 & 6009 &   20 &  4.210 &  0.042 &   0.176 &  0.017 \\ 
  42 &   3616756294553180160 & 5677 &  4.550 &  -0.330 &   3616756294553180288 & 5405 &   24 &  4.560 &  0.044 &  -0.326 &  0.019 \\ 
  43 &   3639520621950395904 & 5997 &  4.450 &  -0.230 &   3639520621950395776 & 5993 &    8 &  4.430 &  0.022 &  -0.233 &  0.008 \\ 
  44 &   3717329177197429376 & 6114 &  4.390 &  -0.021 &   3717329172901660160 & 6232 &   21 &  4.410 &  0.054 &  -0.009 &  0.018 \\ 
  45 &   3749791055416743552 & 5459 &  4.440 &   0.014 &   3749791158495959552 & 5616 &    6 &  4.455 &  0.016 &   0.029 &  0.008 \\ 
  46 &   3759082066110510208 & 6095 &  3.995 &   0.332 &   3759082066110510080 & 6009 &   20 &  3.990 &  0.041 &   0.349 &  0.021 \\ 
  47 &   3830034685322011136 & 6349 &  4.180 &  -0.065 &   3830034479163581312 & 6264 &   37 &  4.050 &  0.063 &  -0.100 &  0.023 \\ 
  48 &    613140808098832000 & 5756 &  4.530 &  -0.034 &   3836997136546164736 & 5936 &   12 &  4.550 &  0.024 &  -0.091 &  0.011 \\ 
  49 &   3898778969789498880 & 6038 &  4.470 &  -0.304 &   3898778901070021504 & 6348 &   21 &  4.430 &  0.056 &  -0.319 &  0.018 \\ 
  50 &   3945118643256370688 & 5398 &  4.550 &  -0.196 &   3945118265299248128 & 5616 &   11 &  4.550 &  0.020 &  -0.178 &  0.008 \\ 
  51 &   3975223065466473216 & 5522 &  4.530 &  -0.174 &   3975129194660883328 & 5656 &    7 &  4.530 &  0.014 &  -0.151 &  0.007 \\ 
  52 &   4024887730814401280 & 6171 &  4.520 &  -0.269 &   4024886425144354816 & 6210 &   16 &  4.450 &  0.044 &  -0.261 &  0.014 \\ 
  53 &   4269938532999515008 & 5828 &  4.210 &  -0.318 &   4104278208452966912 & 6065 &   18 &  4.500 &  0.029 &   0.181 &  0.014 \\ 
  54 &   6643680401021447296 & 5962 &  4.440 &   0.045 &   4174091454408295680 & 5785 &   16 &  4.460 &  0.032 &   0.179 &  0.015 \\ 
  55 &   4193020582174571264 & 6290 &  4.430 &  -0.050 &   4193020582169053056 & 6501 &   18 &  4.330 &  0.037 &  -0.054 &  0.013 \\ 
  56 &   4197023904014523776 & 6079 &  4.550 &  -0.082 &   4197023904013455872 & 5763 &   12 &  4.580 &  0.021 &  -0.067 &  0.011 \\ 
  57 &   4199387544795379968 & 5919 &  4.500 &  -0.082 &   4199387544795378176 & 5923 &    8 &  4.510 &  0.014 &  -0.074 &  0.007 \\ 
  58 &   4235731867269159680 & 6078 &  4.300 &   0.035 &   4235732073427592704 & 6110 &   10 &  4.220 &  0.024 &   0.024 &  0.010 \\ 
  59 &   4240626686883261184 & 5161 &  4.440 &   0.256 &   4240625896609242624 & 5117 &   21 &  4.520 &  0.028 &   0.214 &  0.011 \\ 
  60 &   4249652783985617920 & 5798 &  4.250 &   0.235 &   4249652990144051840 & 5714 &    9 &  4.130 &  0.018 &   0.225 &  0.008 \\ 
  61 &   4499162449416966272 & 6195 &  4.460 &   0.207 &   4287378367995943680 & 6017 &   11 &  4.500 &  0.017 &   0.138 &  0.009 \\ 
  62 &   4343064508746082304 & 5222 &  4.500 &   0.093 &   4343064577465522816 & 5569 &   16 &  4.530 &  0.024 &   0.124 &  0.010 \\ 
  63 &   4360581000283303936 & 5770 &  4.540 &  -0.110 &   4360581000283303552 & 5884 &   10 &  4.530 &  0.019 &  -0.122 &  0.009 \\ 
  64 &   6236816675902817536 & 5626 &  4.460 &  -0.093 &   4383238052280567680 & 6088 &   13 &  4.490 &  0.025 &   0.003 &  0.012 \\ 
  65 &   1198060172076731520 & 5786 &  4.550 &  -0.069 &   4421376193636525184 & 5590 &   15 &  4.540 &  0.027 &  -0.027 &  0.014 \\ 
  66 &   4461273278722817792 & 5328 &  4.450 &   0.074 &   4461273072564386816 & 5614 &   13 &  4.490 &  0.021 &   0.080 &  0.015 \\ 
  67 &   4464207428577214464 & 5443 &  4.520 &  -0.010 &   4464207428579939840 & 5390 &    8 &  4.500 &  0.012 &  -0.018 &  0.006 \\ 
  68 &   4648549830108994816 & 6323 &  4.440 &  -0.171 &   4648549830108995200 & 6347 &   31 &  4.460 &  0.068 &  -0.097 &  0.023 \\ 
  69 &   4666907551119833984 & 6000 &  4.250 &   0.217 &   4666907516760096512 & 6056 &    7 &  4.320 &  0.018 &   0.156 &  0.007 \\ 
  70 &   4677970179988001280 & 6020 &  4.575 &  -0.021 &   4677970179987090304 & 5864 &   21 &  4.520 &  0.038 &  -0.044 &  0.018 \\ 
  71 &   4803965455094278528 & 5991 &  4.460 &  -0.043 &   4805634616824440192 & 5773 &   21 &  4.410 &  0.052 &  -0.017 &  0.022 \\ 
  72 &   4867855155206070784 & 5311 &  4.460 &  -0.072 &   4813691219557127808 & 5706 &   14 &  4.350 &  0.042 &  -0.094 &  0.015 \\ 
  73 &   4837828175549438080 & 6048 &  4.490 &  -0.194 &   4837828179846041728 & 5985 &   20 &  4.520 &  0.034 &  -0.191 &  0.015 \\ 
  74 &   4857866023347844608 & 6036 &  4.490 &  -0.157 &   4857866019051550976 & 6318 &   19 &  4.420 &  0.048 &  -0.081 &  0.017 \\ 
  75 &   4873226853623529856 & 5708 &  4.495 &  -0.037 &   4873223623808123136 & 5766 &   17 &  4.515 &  0.029 &  -0.028 &  0.017 \\ 
  76 &   4940794488850252928 & 6282 &  4.425 &  -0.062 &   4940794866807373952 & 6311 &   13 &  4.355 &  0.031 &  -0.026 &  0.011 \\ 
  77 &   5195685713943687168 & 6124 &  4.455 &  -0.127 &   5195685713943683072 & 6169 &   23 &  4.390 &  0.061 &  -0.176 &  0.016 \\ 
  78 &   5255388783050605824 & 5231 &  4.460 &  -0.088 &   5255388783050603136 & 5237 &   14 &  4.460 &  0.024 &  -0.081 &  0.013 \\ 
  79 &   5296896240321814144 & 5138 &  4.390 &   0.091 &   5296896205962076416 & 5355 &   13 &  4.470 &  0.022 &   0.127 &  0.016 \\ 
  80 &   5401057271783266432 & 6124 &  4.345 &   0.085 &   5401057271781148032 & 6128 &   21 &  4.355 &  0.056 &   0.088 &  0.018 \\ 
  81 &   5484928568505017472 & 6068 &  4.020 &   0.163 &   5484928534145279744 & 6140 &   12 &  4.315 &  0.032 &   0.146 &  0.012 \\ 
  82 &   5485115519841798912 & 5989 &  4.340 &  -0.209 &   5485115588561239808 & 5895 &   10 &  4.410 &  0.029 &  -0.232 &  0.009 \\ 
  83 &   5595858262287843840 & 5802 &  4.230 &   0.107 &   5595858159201264768 & 5625 &    9 &  4.410 &  0.022 &   0.111 &  0.009 \\ 
  84 &   5744680768862271872 & 5917 &  3.840 &   0.139 &   5744680768862271616 & 6329 &   18 &  4.230 &  0.040 &   0.127 &  0.015 \\ 
  85 &   5807733500118617984 & 5723 &  4.530 &   0.196 &   5778002293379364992 & 5478 &   22 &  4.530 &  0.033 &   0.131 &  0.018 \\ 
  86 &   5778208829765876864 & 6019 &  4.350 &  -0.310 &   5778208829765877376 & 5995 &   22 &  4.430 &  0.056 &  -0.324 &  0.018 \\ 
  87 &   5798991008295109120 & 5721 &  4.330 &   0.273 &   5798991008295120896 & 5744 &   13 &  4.270 &  0.027 &   0.276 &  0.013 \\ 
  88 &   5821555284685890304 & 6333 &  4.300 &   0.091 &   5825293319323469824 & 6057 &   14 &  4.220 &  0.031 &   0.014 &  0.012 \\ 
  89 &   5863709946382545280 & 6142 &  4.310 &  -0.120 &   5863709946382541952 & 5920 &   19 &  4.520 &  0.036 &  -0.093 &  0.018 \\ 
  90 &   5877155289930033024 & 5986 &  4.180 &   0.121 &   5877155289930029184 & 5990 &   14 &  4.290 &  0.032 &   0.166 &  0.015 \\ 
  91 &   5897704951769034368 & 6031 &  4.310 &   0.124 &   5897785667103983616 & 6143 &   17 &  4.330 &  0.044 &   0.053 &  0.017 \\ 
  92 &   2598586816173411200 & 6162 &  4.340 &  -0.150 &   5976865876277242112 & 5921 &   13 &  4.290 &  0.035 &  -0.084 &  0.013 \\ 
  93 &   6003429213889816832 & 5971 &  4.490 &   0.091 &   6003429424356691584 & 5630 &   12 &  4.520 &  0.020 &   0.115 &  0.013 \\ 
  94 &   6004256909931771136 & 5353 &  4.430 &   0.138 &   6004256802548180736 & 5480 &   15 &  4.460 &  0.030 &   0.154 &  0.013 \\ 
  95 &   6099322403253174016 & 5639 &  4.550 &   0.075 &   6118406798373150848 & 5540 &   17 &  4.460 &  0.035 &   0.176 &  0.018 \\ 
  96 &   6193279279612173952 & 4986 &  4.420 &  -0.251 &   6193280031230266752 & 4967 &    8 &  4.430 &  0.019 &  -0.234 &  0.008 \\ 
  97 &   6208919660724640896 & 5207 &  4.550 &  -0.080 &   6208919660723526272 & 5345 &   13 &  4.550 &  0.021 &  -0.038 &  0.014 \\ 
  98 &   5906633952564270848 & 5451 &  4.550 &  -0.330 &   6213644846302305536 & 5459 &   13 &  4.500 &  0.020 &  -0.040 &  0.014 \\ 
  99 &   6214634887804201728 & 5938 &  4.520 &  -0.150 &   6214634887804233088 & 5861 &   12 &  4.510 &  0.022 &  -0.160 &  0.009 \\ 
 100 &   6224633983987510528 & 5791 &  4.470 &  -0.270 &   6224633983987511552 & 5851 &   19 &  4.530 &  0.036 &  -0.288 &  0.016 \\ 
 101 &   6274656261191532160 & 6127 &  4.185 &   0.024 &   6274653310550270592 & 6108 &   22 &  4.210 &  0.050 &  -0.061 &  0.015 \\ 
 102 &   6295940298044771072 & 6203 &  4.140 &  -0.198 &   6295940302339553664 & 6372 &   38 &  4.250 &  0.090 &  -0.136 &  0.026 \\ 
 103 &   6317420219765757440 & 6148 &  4.250 &   0.173 &   6317420224061370624 & 6132 &    8 &  4.290 &  0.020 &   0.185 &  0.009 \\ 
 104 &   6369977773223661184 & 5721 &  4.030 &   0.142 &   6369977876303556736 & 6091 &   25 &  4.320 &  0.064 &   0.041 &  0.022 \\ 
 105 &   6740764911228220288 & 5585 &  4.530 &   0.113 &   6381091636756147200 & 5377 &   24 &  4.510 &  0.031 &   0.183 &  0.018 \\ 
 106 &   6463958151650359040 & 5740 &  4.510 &  -0.011 &   6409419145097654016 & 5990 &   22 &  4.500 &  0.035 &  -0.005 &  0.013 \\ 
 107 &   6709875880094622720 & 5712 &  4.540 &  -0.100 &   6420597089545019776 & 5426 &   16 &  4.520 &  0.026 &  -0.106 &  0.017 \\ 
 108 &   6463958151650359040 & 5740 &  4.510 &  -0.011 &   6463958151650358784 & 5634 &   13 &  4.490 &  0.024 &   0.008 &  0.014 \\ 
 109 &   6463958151650358784 & 5621 &  4.530 &  -0.012 &   6463958151650359040 & 5753 &   14 &  4.570 &  0.024 &  -0.012 &  0.014 \\ 
 110 &   6471977542786978688 & 5819 &  4.380 &  -0.472 &   6471977336628547968 & 5363 &   15 &  4.490 &  0.027 &  -0.460 &  0.012 \\ 
 111 &   6473063860275183616 & 6301 &  4.230 &   0.051 &   6472230636619614464 & 6325 &   20 &  4.500 &  0.033 &  -0.006 &  0.014 \\ 
 112 &   6497943781186827264 & 5800 &  4.520 &   0.173 &   6497943781187251072 & 5571 &   15 &  4.530 &  0.024 &   0.086 &  0.015 \\ 
 113 &   6518007050894577664 & 5975 &  4.430 &  -0.050 &   6518006565562564352 & 6065 &   13 &  4.390 &  0.036 &  -0.130 &  0.015 \\ 
 114 &   2328250334633289856 & 5263 &  4.530 &  -0.062 &   6527965258988306304 & 5512 &   14 &  4.500 &  0.021 &   0.055 &  0.012 \\ 
 115 &   6570797524722448896 & 5089 &  4.360 &   0.400 &   6570796871887419648 & 5399 &   21 &  4.410 &  0.045 &   0.394 &  0.022 \\ 
 116 &   6644929416166727680 & 5892 &  4.300 &   0.167 &   6644929656684912512 & 5875 &   12 &  4.340 &  0.032 &   0.123 &  0.012 \\ 
 117 &   6666179333798782976 & 5145 &  4.510 &  -0.160 &   6666179127640352512 & 5120 &   17 &  4.540 &  0.022 &  -0.151 &  0.014 \\ 
 118 &   6673293174030454400 & 5357 &  4.450 &   0.283 &   6673292933512285312 & 5501 &   21 &  4.430 &  0.038 &   0.287 &  0.022 \\ 
 119 &   6673835645579910016 & 5827 &  4.090 &  -0.277 &   6673835611220171904 & 5993 &    8 &  4.390 &  0.020 &  -0.302 &  0.007 \\ 
 120 &   6743004646477330560 & 5335 &  4.510 &   0.000 &   6743004650775553280 & 5210 &   19 &  4.490 &  0.024 &  -0.059 &  0.020 \\ 
 121 &   6805776216277879808 & 5347 &  4.470 &   0.014 &   6805776211983950080 & 5181 &   18 &  4.410 &  0.043 &   0.016 &  0.018 \\ 
 122 &   6827651171911478272 & 5126 &  4.510 &   0.124 &   6827651373773901568 & 5141 &   12 &  4.530 &  0.017 &   0.081 &  0.006 \\ 
 123 &   5767612458250649216 & 6046 &  4.220 &   0.031 &   6866542478736575616 & 6158 &   41 &  4.130 &  0.086 &  -0.209 &  0.023 \\ 
 124 &   6868438517820721152 & 6271 &  4.200 &  -0.364 &   6868432504866186368 & 6132 &   14 &  4.360 &  0.038 &  -0.207 &  0.013 \\ 
 125 &   6900155614347675648 & 6041 &  4.520 &   0.058 &   6889841508084452096 & 6243 &   12 &  4.430 &  0.031 &  -0.059 &  0.012 \\ 
	\hline
	\end{tabular} \\ 
	This table is published in its entirety in the electronic edition of the paper. A portion is shown here for guidance regarding its form and content.
\end{table*}



